Grounded SAM: Assembling Open-World Models for Diverse Visual Tasks

We introduce Grounded SAM, which uses Grounding DINO as an open-set object detector to combine with the segment anything model (SAM). This integration enables the detection and segmentation of any regions based on arbitrary text inputs and opens a door to connecting various vision models. As shown in Fig.1, a wide range of vision tasks can be achieved by using the versatile Grounded SAM pipeline. For example, an automatic annotation pipeline based solely on input images can be realized by incorporating models such as BLIP and Recognize Anything. Additionally, incorporating Stable-Diffusion allows for controllable image editing, while the integration of OSX facilitates promptable 3D human motion analysis. Grounded SAM also shows superior performance on open-vocabulary benchmarks, achieving 48.7 mean AP on SegInW (Segmentation in the wild) zero-shot benchmark with the combination of Grounding DINO-Base and SAM-Huge models.

==> images_tex/automatic-label.tex <==
\begin{figure*}[h]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=0.8\linewidth]{resources/automatic-label.pdf}
    % \vspace{-0.1cm}
    \caption{Automatic Annotation System.}
    \label{fig:automatic_label}
    % \vspace{-0.4cm}
\end{figure*}

==> images_tex/dinobot_overview.tex <==
\begin{figure}[h]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=0.8\linewidth]{resources/dinobot_overview.pdf}
    % \vspace{-0.1cm}
    % \caption{Different modalities can refer}
    \caption{An overview of common modalities includes images in computer vision, which can be further categorized into subsets like box, mask, keypoint, etc, text modality from natural language processing, and audio modality in speech. By mapping these different modalities, various AI capabilities can be achieved.}
    % 
    \label{fig:dinobot_overview}
    \vspace{-0.4cm}
\end{figure}

==> images_tex/grounded_sam_human.tex <==
\begin{figure*}[h]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=0.8\linewidth]{resources/Grounded-SAM-Human.pdf}
    % \vspace{-0.1cm}
    \caption{Combine \textbf{Grounded-SAM} with \textbf{OSX} to link 2D human box with 3D mesh.}
    \label{fig:grounded_sam_human}
    % \vspace{-0.4cm}
\end{figure*}

==> images_tex/grounded_sam_pipeline.tex <==
\begin{figure*}[h]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=0.8\linewidth]{resources/Grounded-SAM-Pipeline.pdf}
    % \vspace{-0.1cm}
    \caption{The pipeline of our Grounded-SAM playground.}
    \label{fig:grounded_sam_pipeline}
    % \vspace{-0.4cm}
\end{figure*}

==> images_tex/grounded_sam_teaser.tex <==
\begin{figure*}[h]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=.9\linewidth]{resources/grounded_sam_overview.pdf}
    % \vspace{-0.1cm}
    \caption{\textbf{Grounded-SAM} has the capability to simultaneously detect and segment corresponding regions within images based on arbitrary text inputs provided by users.}
    \label{fig:grounded_sam_overview}
    % \vspace{-0.4cm}
\end{figure*}

==> images_tex/inpainting.tex <==
\begin{figure*}[h]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=0.8\linewidth]{resources/inpainting.pdf}
    % \vspace{-0.1cm}
    \caption{Combine \textbf{Grounded-SAM} with \textbf{Stable-Diffusion Inpainting} to generate new data.}
    \label{fig:inpainting}
    % \vspace{-0.4cm}
\end{figure*}

==> images_tex/interactive.tex <==
\begin{figure*}[h]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=0.8\linewidth]{resources/interactive.pdf}
    % \vspace{-0.1cm}
    \caption{Combine \textbf{Grounded-SAM} with \textbf{Segment-Anything} to refine the segmentation output.}
    \label{fig:interactive}
    % \vspace{-0.4cm}
\end{figure*}

==> images_tex/reasoning.tex <==
\begin{figure*}[h]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=0.65\linewidth]{resources/reasoning2.pdf}
    % \vspace{-0.1cm}
    \caption{Combine \textbf{Grounded-SAM} with \textbf{ChatGPT} to perform multi-modal reasoning.}
    \label{fig:reasoning}
    % \vspace{-0.4cm}
\end{figure*}

==> images_tex/semi-automatic-label-system.tex <==
\begin{figure*}[h]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=0.8\linewidth]{resources/semi-automatic-label-system.pdf}
    % \vspace{-0.1cm}
    \caption{Semi-automatic Annotation System. We also regard it as the basic architecture of \textbf{Grounded-SAM}}
    \label{fig:semi_automatic_annotation_system}
    % \vspace{-0.4cm}
\end{figure*}

==> sections/01_intro.tex <==
\section{Introduction}


% \input{images_tex/dinobot_overview}

\begin{figure*}[h]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=.9\linewidth]{resources/grounded_sam_overview.pdf}
    % \vspace{-0.1cm}
    \caption{\textbf{Grounded-SAM} has the capability to simultaneously detect and segment corresponding regions within images based on arbitrary text inputs provided by users.}
    \label{fig:grounded_sam_overview}
    % \vspace{-0.4cm}
\end{figure*}





Visual perception and understanding tasks in open-world scenarios hold vast potential for applications such as autonomous driving, robotic navigation, and intelligent security surveillance. These applications set stringent demands on the visual perception capabilities of models. Currently, three primary approaches are employed to address the challenges of visual perception in open contexts: 1. \textbf{Unified Model}: Models like GPT-4v~\cite{openai2023gpt4} and LLaVA~\cite{llava} are examples of multimodal large language models (MLLM) which, by incorporating visual modality on top of the standard large language models, extend the capacity of LLMs to encompass visual tasks in open contexts. 2. \textbf{LLM as Controller}: Approaches like HuggingGPT~\cite{shen2023hugginggpt} and Visual ChatGPT~\cite{visualchatgpt} utilize the linguistic comprehension of LLMs. Given textual inputs, which define tasks and conditions, the LLMs direct various agent models to address complex visual tasks within diverse scenarios. 3. \textbf{Ensemble Foundation Model}: Achieving open-world tasks in complex scenarios by collaboratively integrating expert models designed for singular contexts. 
% 感觉这里可以加一个过渡，"我们Grounded-SAM在第三条赛道上是比较典型的代表"



% Taking the fundamental computer vision perception tasks (e.g., object detection, segmentation, and human pose estimation)~\cite{zhang2022dino,li2023maskdino,lin2023osx,yang2023explicit} as example, the more generalizable Open-Vocabulary Perception Models~\cite{liu2023grounding, zhang2023simple, yang2023unipose} is receiving increasing attention. As the field moves towards addressing broader challenges, open-world segmentation tasks stand out as representative challenges. 

%
Current models have achieved remarkable performance on modality mapping tasks by constantly improving model designs \cite{he2015deep, Radford2021LearningTV,liu2023grounding,ren2023strong}, training methods \cite{DiederikPKingma2014AdamAM,gozalo2023chatgpt}, and expanding datasets \cite{schuhmann2022laion,schuhmann2021laion,ju2023humansd}.  Despite significant progress in addressing modality-to-modality mapping challenges, lots of challenges still exist in complex cases. For instance, the open-set segmentation problem, which involves segmenting unseen objects in open-world scenarios, remains difficult to solve. It can be viewed as a text-to-mask mapping problem, with one reason for its difficulty being the lack of high-quality annotated data.
% 
Recently, SAM~\cite{kirillov2023segment} introduces an interactive segmentation model trained on a large dataset with only mask annotations. However, this approach imposes limitations on its capability to effectively map between texts and masks, such as precise segmentation of corresponding regions based on a user's text prompt.

Although establishing a direct modality mapping from text to mask is a highly complex task, mapping from text to box and from box to mask is comparatively simpler.
Mapping text to box involves simply locating the region-level bounding box corresponding to an object described in the text, which is comparatively simpler than generating a pixel-level mask. Similarly, box-to-mask mapping primarily entails refining the bounding box to align with the object's shape, which is also a less challenging task compared to generating a mask from scratch. Moreover, text-to-box and box-to-mask mappings benefit from more extensive data sources, such as object detection \cite{shao2019objects365} and segment anything \cite{kirillov2023segment} datasets. However, text-to-mask mapping problems face challenges due to the scarcity of data specifically annotated with masks for corresponding text queries. This annotation process is more costly and time-consuming, contributing to the limited availability of high-quality training data.
% 

Despite the current underperformance of models in directly tackling the text-to-mask task, some works have achieved good results in the comparatively simpler tasks of text-to-box and box-to-mask mappings.
For example, Grounded Pre-training \cite{li2021grounded, liu2023grounding} provides a large amount of training data for the text-to-box mapping problem, and SAM can perform the box-to-mask mapping well. This inspires us to solve complex modality mapping problems by \textbf{assembling} different foundation models\footnote{We use the term "foundation models" here for pre-trained and API-well-defined models in this paper. We do not care about the model scale or training data scale.}. We term the idea of assembling foundation models into \textbf{DinoBot}. Each model functions akin to the disparate parts of a DinoBot, each bearing unique characteristics and capabilities. When they work collaboratively, being pieced together into a fully-formed DinoBot, they manifest collective strength and intelligence, capable of addressing more complex tasks.


To verify this concept, we develop a framework called \textbf{Grounded-SAM} to address the text-to-mask mapping problem. It assembles Grounding-DINO \cite{liu2023grounding} with SAM \cite{kirillov2023segment}. Grounded-SAM firstly utilizes Grounding-DINO to detect objects based on human inputs, and then generate masks conditioned on the boxes with SAM. Grounded-SAM can segment unseen objects in open-world scenarios with natural language queries. It solves the text-to-mask mapping problem effectively. 
% 
In addition, by building upon the foundation of Grounded-SAM, we can incorporate various other expert models, including BLIP~\cite{li2022blip}, Stable-Diffusion~\cite{rombach2022high}, ChatGPT~\cite{gozalo2023chatgpt}, OSX~\cite{lin2023osx}, etc., allowing us to construct a diverse range of powerful AI systems to fulfill the basic requirements, including understanding, generation, interactive, and reasoning.

% we assemble Grounded-SAM with various cross-modal components, like BLIP \cite{li2022blip}, Whisper \cite{whisper}, ChatGPT \cite{gozalo2023chatgpt}, OSX~\cite{lin2023osx}, etc., which enables the model to obtain all four basic abilities.
Our contributions can be summarized as follows:
\begin{enumerate}
    \item We propose the concept of DinoBot, which involves integrating different expert models sequentially to accomplish complex modality mapping artificial intelligence tasks.
    \item We construct several specific applications to validate the effectiveness of the DinoBot concept. For instance, to address the complex text-to-mask task, we combine the Grounding-DINO model, which excels in text-to-box mapping, with the SAM model, which performs well in box-to-mask mapping. By integrating these models, we effectively address the open-set segmentation task (mapping from text to mask).
    \item Building upon the framework of Grounded-SAM, we further incorporate more models to achieve a wide range of advanced artificial intelligence applications.
\end{enumerate}






